Improved Algorithms for Contextual Dynamic Pricing

In contextual dynamic pricing, a seller sequentially prices goods based on contextual information. Buyers will purchase products only if the prices are below their valuations. The goal of the seller is to design a pricing strategy that collects as much revenue as possible. We focus on two different valuation models. The first assumes that valuations linearly depend on the context and are further distorted by noise. Under minor regularity assumptions, our algorithm achieves an optimal regret bound of $\tilde{\mathcal{O}}(T^{2/3})$, improving the existing results. The second model removes the linearity assumption, requiring only that the expected buyer valuation is $\beta$-H\"older in the context. For this model, our algorithm obtains a regret $\tilde{\mathcal{O}}(T^{d+2\beta/d+3\beta})$, where $d$ is the dimension of the context space.

==> AlgorithmicApproach.tex <==
\section{Algorithmic Approach -- Valuation Approximation - Price Elimination}

In this section, we present the general algorithmic approach that we use to tackle dynamic pricing with covariates, called \textsc{Valuation Approximation - Price Elimination (VAPE)}. Before presenting the full scheme, we start with some intuition that leads to its design.

% The intuition behind our approach comes from \Cref{eq: revenue for demand increments}. 
Assume for a moment that we have full knowledge of the valuation function $g$. Then, by \Cref{eq: revenue for demand increments}, the only uncertainty in the expected reward is due to the demand function $D$ at the price increment $\delta$. Now, let $\brc*{\delta_k}_{k\in\cK}$ be a set of candidate price increments and assume we set a price $p_t=g(x_t)+\delta_k$. Then, the observation $o_t$ of whether a trade took place can be used to estimate the demand, since
\begin{align*}
    \E{o_t} = \E{\indicator{g(x_t)+\xi_t\ge g(x_t)+\delta_k}} = D(\delta_k).
\end{align*}
In particular, letting $\widehat{D}^k_t$ be the empirical probability of a trade when playing a price increment $\delta_k$ based on samples before time $t$, one could use standard bandit arguments to estimate the demand such that w.h.p.,
\begin{align*}
    D(\delta_k)\in\brs*{\widehat{D}^k_t - \sqrt{\frac{2\log(\nicefrac{1}{\delta})}{N_t^k}}, \widehat{D}^k_t +\sqrt{\frac{2\log(\nicefrac{1}{\delta})}{N_t^k}}},
\end{align*}
where $N_t^k$ is the number of times a price increment $\delta_k$ was played before time $t$. Using \Cref{eq: revenue for demand increments}, one can readily use these estimators to also build confidence intervals for the rewards and achieve favorable regret using a successive elimination algorithm \citep{JMLR:v7:evendar06a,perchet2013multi}. More precisely, we suggest sampling non-eliminated increments in a round-robin fashion while using the confidence bound to gradually eliminate increments. We term this part of the algorithm as \textsc{Price Elimination}.

However, in practice, we do not know the exact valuation of a context $x_t$ and only have its estimate, which we denote by $\widehat{g}_t$. Using this estimate to set a price $p_t=\widehat{g}_t + \delta$ effectively creates a small error in the price increment we aim to set:
\begin{align*}
    \pi(x_t, p_t)
    = \pi\br*{x_t, g(x_t) + \br*{\delta + \widehat{g}_t - g(x_t)} }
    = \br*{g(x_t) + \br*{\delta + \Delta g_t}} \times D\br*{\delta + \Delta g_t}.
\end{align*}
for $\Delta g_t=\widehat{g}_t - g(x_t)$.
Luckily, since the demand is Lipschitz in the price increment, as long the error $\Delta g_t$ is small, the biased demand $\delta + \Delta g_t$ will yield a similar reward to the desired price $g(x_t)+\delta$. The goal of the \textsc{Valuation Approximation} is to accurately approximate $g(x_t)$. To do so, we rely on the following remark: when the price $p_t$ is uniformly chosen from the interval $[-B_y,B_y]$, the random variable $2B_y\left(o_t-1/2\right)$ serves as an unbiased estimate of $g(x_t)$ conditioned on $x_t$. Given that $2B_y\left(o_t-1/2\right)$ is bounded, classical concentration results can be employed to bound the error of our estimates for $g(x_t)$.

At each round, we test whether our estimate of $g(x_t)$ is precise enough to ensure that the error $\Delta g_t$ is small compared to the error term $\sqrt{\nicefrac{2\log(\nicefrac{1}{\delta})}{N_t^k}}$. If this is the case, we proceed with the \textsc{Price Elimination} subroutine; otherwise, we conduct another \textsc{Valuation Approximation} round. In the following Section, we discuss how to bound the number of valuation approximation rounds is limited. Moreover, we show how to correct both the demand and reward confidence intervals to accommodate for the approximation error $\Delta g_t$.
%Given error level $\mu>0$ and assuming an error bound $\Delta g_t\le \textnormal{CB}_t(x_t)$ (derived using concentration bounds depending on the structure of $g$), we test whether $\textnormal{CB}_t(x_t)\le \mu$. If this is the case, we continue to the price elimination for this context; otherwise, we improve our valuation estimator by setting a uniform price $p_t \sim \cU([-B_y,B_y])$. We will later prove that this allows extracting an unbiased estimator of the valuation $g(x_t)$ and that for both linear and nonparametric valuations, the number of valuation approximation rounds is limited. Moreover, we show how to correct both the demand and reward confidence intervals to accommodate for the approximation error $\mu$. \sol{I think we should put more emphasis on how estimating the prices this way from binary feedbacks is novel. Not that it is that difficult, but it's clearly more clever than what was done previously. I'll write something.} \nadav{sure :-)}
The high-level algorithmic scheme is described in \Cref{alg:high-level}. 

\begin{algorithm}[t]
\caption{Valuation Approximation - Price Elimination (VAPE) General scheme}\label{alg:high-level}
\begin{algorithmic}[1]
\State \textbf{Input}: Price increments $\brc*{\delta_k}_{k\in\cK}$, valuation confidence $\textnormal{CB}_t(x)$, reward confidence intervals $[\LCB_t(k),\UCB_t(k)]$, parameters $\delta$, $\mu$.
%%%
\While{$t \leq T$}
\If{$\textnormal{CB}_t(x) > \mu$} \Comment{Valuation Approximation}
    \State Post price $p_t \sim \cU([-B_y,B_y])$
    \State Use $o_t$ to improve the valuation estimator $\widehat{g}(x)$
\Else \Comment{Price Elimination}
\State  $\cA_t \gets \Bigg\{k \in \cK : \widehat{g}_t + \delta_k \in [0,B_y]\Bigg\}$
\State $\cK_t \gets \{k \in \cA_t : \UCB_t(k) \geq \max_{k'\in \cA_t} \LCB_t(k')\}$
\State Choose $k_t \in \argmin_{k \in \cK_t}  N_t^{k}$, post price $p_t = \widehat{g}_t + \delta_{k_t}$
\State Update $\widehat{D}_{t+1}^{k_t}$, $N_t^{k_t}$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

We underline that while the subroutine for estimating valuations $g(x_t)$ for binary feedback is relatively straightforward, and the associated errors are easily bounded using classical concentration results, it is to the best of the author's knowledge the first time that this method was used in dynamic pricing. Previous approaches for estimating valuation functions in the linear valuation model include, among others, the regularized maximum-likelihood estimator \citep{javanmard2019dynamic, wang2023online}, which, however, requires knowledge of the noise distribution. Another approach introduced by \cite{luo2024distribution} relies on the relationship between the problem of estimating a linear valuation function from binary feedback, and the classical linear classification problem, by emphasizing that a sale occurs at price $p_t$ with a probability greater than $1/2$ if and only if $x_t^{\top}\theta - p_t + F^{-1}(1/2) > 0$. The authors propose recovering the parameter $\theta$ through logistic regression; however, they do not provide an explicit estimation rate for $\theta$. On the other hand, \cite{liu2021optimal} utilize the \textsc{EXP-4} algorithm to aggregate policies corresponding to different values of $\theta$ and $F$, thus circumventing the necessity to estimate them. In a similar vein, in the non-parametric valuation model, \cite{chen2021nonparametric} avoid the need to estimate the non-parametric reward $g(x_t)$ by employing independent bandit algorithms for each (binned) value of $x_t$. Closer to our method, \cite{fan2024policy} also employ uniform prices to obtain unbiased estimates of valuations. However, their analysis is more intricate and necessitates stronger assumptions regarding the c.d.f. of the noise and the distribution of the contexts.

In the following sections, we prove that \textsc{VAPE} achieves order-optimal regret for linear valuations and improved regret for non-parametric valuations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\sol{I am trying smth here}

